[EDGE] A grouped calibration test for logistic regression that tolerates a few corrupted records

The Hosmer-Lemeshow calibration test groups patients by predicted risk for a valid reference and loses power that more groups cannot recover. Later tests weight each record's residual alone, which makes them fragile: on an otherwise correct model, one record in a thousand with a corrupted covariate raises the false-alarm rate of Stukel's score test from 5% to 12%, and ten to 63%. Pooling on equal-size groups bounds a wrong record's influence, dividing its residual by its groupmates' variance; without pooling, the same directions are as fragile as Stukel's test after a refit. EDGE, the test proposed here, projects the grouped residuals onto a small basis of calibration shapes. Its degrees of freedom do not depend on the number of groups, so the partition becomes a setting, fine-grained for power and coarse when records may be wrong, and its reference needs no resampling. In a prespecified simulation EDGE was comparable in power to Stukel's test on clean data and 0.064 more powerful on average than the ten-group Hosmer-Lemeshow test. With one and ten exaggerated covariates in a thousand its false-alarm rates were 0.056 and 0.097, and with ten groups below 0.10 up to about ten exaggerated or five reversed. In external validation, at ten groups, its average power was that of Cox's recalibration test and the GiViTI belt, and its false-alarm rate stayed below 0.10 with ten reversed records in a thousand, where theirs did not. In a 70,000-patient cohort its verdict did not change with the partition.

==> tables/tab_contamination.tex <==
\begin{table}[tp]\centering\small
\caption{False-alarm rate at the nominal $5\%$ level when $k$ records carry a corrupted
covariate and the model is correct for every other record; the $k=0$ rows are sizes on the same
design. $1000$ replicates a scenario; the nominal standard error is $0.007$. EDGE is in its
unit form at the default partition, with the cubic (default) and symmetric bases, and the
Hosmer--Lemeshow statistic is shown at both partitions. The pooled tests combine each record's
residual with those of other records --- in groups of predicted risk, or for le Cessie's test
over neighbourhoods in covariate space. Every test built on each record's own
linear predictor rises with $k$. The last two rows give the median time a data set in milliseconds on
one core (the symmetric forms were not timed). Le Cessie's test is protected but holds an $n\times n$
kernel and grows with the cube of $n$; it was run with corrupted records at $n=1000$ only.}
\label{tab:contamination}
\resizebox{\textwidth}{!}{\begin{tabular}{rrrrrrrrrrr}\hline
 & & \multicolumn{5}{c}{pooled} & \multicolumn{4}{c}{record-level} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-11}
$n$ & $k$ & EDGE & EDGE-sym & HL ($G$ rule) & HL ($G{=}10$) & le Cessie & Stukel joint & Stukel sym & GiViTI & cubic LR \\ \hline
1000 & 0 & 0.045 & 0.044 & 0.038 & 0.040 & 0.059 & 0.044 & 0.049 & 0.042 & 0.041 \\
1000 & 1 & 0.056 & 0.058 & 0.052 & 0.051 & 0.055 & 0.121 & 0.115 & 0.089 & 0.127 \\
1000 & 2 & 0.059 & 0.067 & 0.051 & 0.044 & 0.052 & 0.217 & 0.206 & 0.146 & 0.201 \\
1000 & 5 & 0.057 & 0.048 & 0.045 & 0.042 & 0.052 & 0.398 & 0.367 & 0.251 & 0.321 \\
1000 & 10 & 0.097 & 0.059 & 0.066 & 0.058 & 0.077 & 0.627 & 0.592 & 0.397 & 0.482 \\
5000 & 0 & 0.048 & 0.053 & 0.052 & 0.055 & -- & 0.047 & 0.052 & 0.048 & 0.041 \\
5000 & 5 & 0.050 & 0.045 & 0.043 & 0.037 & -- & 0.252 & 0.222 & 0.187 & 0.272 \\
5000 & 10 & 0.060 & 0.052 & 0.052 & 0.043 & -- & 0.472 & 0.420 & 0.312 & 0.447 \\
5000 & 25 & 0.151 & 0.099 & 0.077 & 0.050 & -- & 0.801 & 0.784 & 0.575 & 0.753 \\
5000 & 50 & 0.740 & 0.745 & 0.437 & 0.088 & -- & 0.980 & 0.977 & 0.869 & 0.954 \\
\hline
\multicolumn{2}{l}{ms, $n=1000$} & 4 & -- & 2 & 2 & 5,570 & 1 & -- & 9 & 5 \\
\multicolumn{2}{l}{ms, $n=5000$} & 14 & -- & 7 & 7 & 1,267,530 & 2 & -- & 33 & 19 \\
\hline\end{tabular}}\end{table}


==> tables/tab_edgefr.tex <==
\begin{table}[htbp]\centering\small
\caption{The tail-pooled setting EDGE-FR, at three tail fractions, against the default partition and
against ten groups. Its default column repeats the EDGE column of
Table S5 for the eight scenarios the two tables share, so that the
comparison can be read in place. EDGE-FR$(c)$ puts the outer $5c$ of the risk scale at each end into one group
and leaves the middle at the default partition, which is used throughout otherwise. $1000$ replicates
a scenario, the same data sets for every setting. The false alarms are rejection rates at the
nominal $5\%$ level under a correct logistic model with $k$ records carrying a corrupted
covariate; the rows at $k \ge 20$ for $n=1000$ and $k \ge 100$ for $n=5000$ were run on fresh
seeds, whose uncontaminated scenarios read between
$0.034$ and $0.062$ for every setting. The power rows are size-adjusted, each setting at its own
critical value read from the matched null scenario, and the first is the mean over six link and
tail scenarios at $n=1000$ (cauchit, log--log, three Stukel designs, $t_4$); the paired readings behind them are in the
archive. Widening the tails costs power without adding protection in proportion, and the
protection ends in every setting once the corrupted records pass a few tens.}
\label{tab:edgefr}
\begin{tabular}{lrrrrr}\hline
 & & \multicolumn{3}{c}{EDGE-FR} & \\
\cmidrule(lr){3-5}
Scenario & default & $c=1\%$ & $c=2\%$ & $c=4\%$ & ten groups \\ \hline
\multicolumn{6}{l}{\emph{false alarms, $k$ records with a corrupted covariate}} \\
\quad $n=1000$, $k=1$ & 0.056 & 0.064 & 0.059 & 0.056 & 0.056 \\
\quad $n=1000$, $k=2$ & 0.059 & 0.053 & 0.049 & 0.048 & 0.053 \\
\quad $n=1000$, $k=5$ & 0.057 & 0.047 & 0.053 & 0.056 & 0.051 \\
\quad $n=1000$, $k=10$ & 0.097 & 0.081 & 0.079 & 0.050 & 0.085 \\
\quad $n=1000$, $k=20$ & 0.227 & 0.140 & 0.104 & 0.100 & 0.101 \\
\quad $n=1000$, $k=40$ & 0.714 & 0.397 & 0.226 & 0.169 & 0.234 \\
\quad $n=5000$, $k=5$ & 0.050 & 0.041 & 0.043 & 0.052 & 0.048 \\
\quad $n=5000$, $k=10$ & 0.060 & 0.045 & 0.045 & 0.055 & 0.047 \\
\quad $n=5000$, $k=25$ & 0.151 & 0.059 & 0.059 & 0.056 & 0.065 \\
\quad $n=5000$, $k=50$ & 0.740 & 0.111 & 0.113 & 0.097 & 0.107 \\
\quad $n=5000$, $k=100$ & 1.000 & 0.431 & 0.338 & 0.246 & 0.328 \\
\quad $n=5000$, $k=200$ & 1.000 & 0.987 & 0.956 & 0.863 & 0.945 \\
\multicolumn{6}{l}{\emph{level, no corruption}} \\
\quad $n=1000$ & 0.045 & 0.039 & 0.043 & 0.050 & 0.040 \\
\quad $n=5000$ & 0.048 & 0.050 & 0.041 & 0.048 & 0.051 \\
\multicolumn{6}{l}{\emph{power against a real misfit}} \\
\quad six link and tail scenarios, mean & 0.500 & 0.490 & 0.449 & 0.408 & 0.483 \\
\quad complementary log--log, $n=1000$ & 0.826 & 0.824 & 0.778 & 0.662 & 0.812 \\
\quad probit, $n=5000$ & 0.278 & 0.239 & 0.196 & 0.146 & 0.223 \\
\hline\end{tabular}\end{table}


==> tables/tab_external.tex <==
\begin{table}[htbp]\centering\small
\caption{External validation: a published model with frozen coefficients checked on new patients. Five
standard normal covariates; the truth departs from the published linear predictor in five ways, two
strengths each, at $n=500$; in the last block the model is correct and $k$ of $1000$ records carry the
second covariate multiplied by four (exaggeration) or by $-4$ (sign error), with their prediction
recomputed at the recorded value. EDGE is in external mode (cubic basis and constant, four
degrees of freedom) at ten groups and at the default partition. Cox is the recalibration test on
intercept and slope, Spiegelhalter the $z$ test, GiViTI the belt in external mode, HL the
Hosmer--Lemeshow statistic at ten groups and Stukel his two terms added to the frozen linear predictor.
$1000$ replicates a scenario. Power is size-adjusted at the null with $n=500$; shaded false-alarm rates
exceed $0.10$.}
\label{tab:external}
\resizebox{\textwidth}{!}{\begin{tabular}{lrrrrrrr}\hline
Scenario & EDGE, $G{=}10$ & EDGE, default & Cox & Spiegelhalter & GiViTI & HL & Stukel \\ \hline
\multicolumn{8}{l}{\emph{Level: rejection rate of a correct model}} \\
\quad $n=250$ & 0.051 & 0.051 & 0.053 & 0.050 & 0.056 & 0.048 & 0.051 \\
\quad $n=500$ & 0.051 & 0.054 & 0.055 & 0.057 & 0.053 & 0.052 & 0.062 \\
\quad $n=1000$ & 0.061 & 0.050 & 0.061 & 0.061 & 0.060 & 0.048 & 0.052 \\
\multicolumn{8}{l}{\emph{Power, size-adjusted, $n=500$}} \\
\quad calibration in the large, $C=0.2$ & 0.311 & 0.298 & 0.390 & 0.107 & 0.392 & 0.216 & 0.153 \\
\quad calibration in the large, $C=0.4$ & 0.911 & 0.894 & 0.953 & 0.303 & 0.951 & 0.770 & 0.493 \\
\quad calibration slope, $C=0.8$ & 0.394 & 0.387 & 0.415 & 0.526 & 0.415 & 0.290 & 0.321 \\
\quad calibration slope, $C=0.6$ & 0.972 & 0.971 & 0.987 & 0.994 & 0.987 & 0.929 & 0.956 \\
\quad U-shaped term, $C=0.4$ & 0.124 & 0.127 & 0.079 & 0.075 & 0.084 & 0.104 & 0.084 \\
\quad U-shaped term, $C=0.8$ & 0.460 & 0.470 & 0.342 & 0.271 & 0.361 & 0.335 & 0.322 \\
\quad threshold term, $C=2$ & 0.135 & 0.120 & 0.203 & 0.067 & 0.202 & 0.102 & 0.163 \\
\quad threshold term, $C=4$ & 0.277 & 0.240 & 0.418 & 0.086 & 0.429 & 0.161 & 0.282 \\
\quad interaction, $C=0.6$ & 0.144 & 0.151 & 0.091 & 0.072 & 0.102 & 0.115 & 0.103 \\
\quad interaction, $C=1$ & 0.424 & 0.459 & 0.218 & 0.210 & 0.279 & 0.332 & 0.390 \\
\quad mean of the ten & 0.415 & 0.412 & 0.410 & 0.271 & 0.420 & 0.335 & 0.327 \\
\multicolumn{8}{l}{\emph{False alarms, correct model, $n=1000$}} \\
\quad exaggeration, $k=1$ & 0.044 & 0.055 & 0.054 & 0.048 & 0.055 & 0.040 & 0.048 \\
\quad exaggeration, $k=2$ & 0.034 & 0.043 & 0.046 & 0.043 & 0.047 & 0.046 & 0.070 \\
\quad exaggeration, $k=5$ & 0.059 & 0.072 & 0.050 & 0.054 & 0.063 & 0.048 & \cellcolor{black!12}0.123 \\
\quad exaggeration, $k=10$ & 0.055 & 0.077 & 0.072 & 0.070 & 0.089 & 0.064 & \cellcolor{black!12}0.173 \\
\quad sign error, $k=1$ & 0.045 & 0.040 & 0.043 & 0.047 & 0.057 & 0.050 & \cellcolor{black!12}0.114 \\
\quad sign error, $k=2$ & 0.044 & 0.051 & 0.043 & 0.044 & 0.080 & 0.058 & \cellcolor{black!12}0.132 \\
\quad sign error, $k=5$ & 0.065 & \cellcolor{black!12}0.104 & 0.088 & 0.071 & \cellcolor{black!12}0.192 & 0.067 & \cellcolor{black!12}0.349 \\
\quad sign error, $k=10$ & 0.082 & \cellcolor{black!12}0.240 & \cellcolor{black!12}0.158 & 0.090 & \cellcolor{black!12}0.347 & 0.076 & \cellcolor{black!12}0.610 \\
\quad settings held, of eight & 8 & 6 & 7 & 8 & 6 & 8 & 2 \\
\hline\end{tabular}}\end{table}


==> tables/tab_hypotheses.tex <==
\begin{table}[htbp]\centering\small
\caption{The seven hypotheses declared before the study was run, and their outcomes. The
statistic and the threshold are those fixed in the pre-declaration; no threshold was moved after
the results were seen.}
\label{tab:hypotheses}
\vspace{4pt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}l>{\raggedright\arraybackslash}p{0.30\textwidth}rrrll@{}}\toprule
Hypothesis & Statement & Scenarios & Statistic & Threshold & Outcome & Leads or ties$^{a}$ \\ \midrule
H1 & EDGE-poly3 leads GiViTI on symmetric tails & 32 & 0.105 & 0.1 & \textbf{against} & 26 of 32 \\
H2 & EDGE-sym is not behind Stukel's joint score & 32 & 0.005 & $-0.014$ & \textbf{holds} & 25 of 32 \\
H3 & EDGE-poly3 is not far behind GiViTI on asymmetric links & 21 & $-0.075$ & $-0.05$ & \textbf{against} & 7 of 21 \\
H4 & EDGE-poly3 leads or ties the partition tests at $G=10$ & 29 & 17 & 19 & \textbf{against} & 17 of 19 \\
H4-ruleG & the same at the default partition & 29 & 21 & 19 & reported & 21 of 21 \\
H5 & EDGE-sym is not behind Stukel's one-parameter score & 4 & 0.006 & 0.02 & \textbf{holds} & 2 of 4 \\
H5-skew & the same under a skewed covariate & 4 & 0.252 & -- & reported & 0 of 4 \\
\bottomrule\end{tabular}
\par\smallskip\parbox{\textwidth}{\footnotesize $^{a}$Scenarios in which EDGE leads or ties within $0.01$:
a description, not the declared test. The two can differ: H1 fails its declared condition on one
design while EDGE leads or ties in $26$ of $32$ scenarios. Section 5.2 of the main text reports
the outcomes as findings.}
\end{table}


==> tables/tab_pairedfam.tex <==
\begin{table}[htbp]\centering\small
\caption{Mean difference in size-adjusted power, EDGE (cubic basis, unit form, default partition) minus
each comparator, by departure family, with a Monte Carlo $95\%$ interval in brackets. The interval
ignores the positive correlation between two tests read on the same replicates, which makes it
conservative, and the Monte Carlo error of the critical values used for size adjustment. The last
column is the price of ten groups.}
\label{tab:pairedfam}
\resizebox{\textwidth}{!}{\begin{tabular}{lrllllll}\hline
Family & Scenarios & HL, ten groups & Stukel joint & Stukel one-par. & cubic LR & GiViTI & EDGE, ten groups \\ \hline
symmetric tails & 32 & $+0.175$ {\footnotesize(0.171, 0.179)} & $-0.007$ {\footnotesize(-0.011, -0.003)} & $-0.062$ {\footnotesize(-0.066, -0.058)} & $+0.001$ {\footnotesize(-0.003, 0.005)} & $+0.105$ {\footnotesize(0.101, 0.109)} & $+0.036$ {\footnotesize(0.032, 0.040)} \\
asymmetric links & 21 & $+0.183$ {\footnotesize(0.180, 0.187)} & $-0.010$ {\footnotesize(-0.014, -0.006)} & $+0.183$ {\footnotesize(0.179, 0.187)} & $-0.072$ {\footnotesize(-0.076, -0.068)} & $-0.075$ {\footnotesize(-0.079, -0.071)} & $+0.024$ {\footnotesize(0.020, 0.028)} \\
Stukel symmetric family & 10 & $+0.127$ {\footnotesize(0.123, 0.131)} & $-0.002$ {\footnotesize(-0.006, 0.002)} & $-0.054$ {\footnotesize(-0.058, -0.050)} & $-0.022$ {\footnotesize(-0.026, -0.018)} & $+0.107$ {\footnotesize(0.103, 0.111)} & $+0.019$ {\footnotesize(0.015, 0.023)} \\
omitted terms & 80 & $+0.067$ {\footnotesize(0.066, 0.069)} & $-0.015$ {\footnotesize(-0.017, -0.014)} & $-0.026$ {\footnotesize(-0.027, -0.025)} & $+0.010$ {\footnotesize(0.008, 0.011)} & $-0.022$ {\footnotesize(-0.023, -0.020)} & $+0.011$ {\footnotesize(0.009, 0.012)} \\
rough misfit & 13 & $-0.461$ {\footnotesize(-0.464, -0.458)} & $-0.008$ {\footnotesize(-0.012, -0.004)} & $-0.038$ {\footnotesize(-0.042, -0.034)} & $-0.023$ {\footnotesize(-0.027, -0.020)} & $+0.093$ {\footnotesize(0.089, 0.097)} & $-0.000$ {\footnotesize(-0.004, 0.003)} \\
off-index & 2 & $+0.026$ {\footnotesize(0.019, 0.034)} & $-0.002$ {\footnotesize(-0.010, 0.006)} & $+0.031$ {\footnotesize(0.024, 0.038)} & $+0.001$ {\footnotesize(-0.007, 0.009)} & $-0.007$ {\footnotesize(-0.016, 0.001)} & $+0.018$ {\footnotesize(0.010, 0.025)} \\
all families & 158 & $+0.064$ {\footnotesize(0.063, 0.066)} & $-0.011$ {\footnotesize(-0.013, -0.010)} & $-0.007$ {\footnotesize(-0.009, -0.006)} & $-0.008$ {\footnotesize(-0.009, -0.007)} & $+0.015$ {\footnotesize(0.014, 0.016)} & $+0.017$ {\footnotesize(0.016, 0.018)} \\
\hline\end{tabular}}\end{table}


==> tables/tab_rivals_contam.tex <==
\begin{table}[htbp]\centering\small
\caption{False-alarm rate at the nominal $5\%$ level when three records of $n=500$ have their
covariate multiplied by four or by eight and the model is correct for every other record. $100$
replicates a scenario, every test on the same data sets; the nominal standard error is $0.022$. EDGE is
in its unit form at the default partition, which is twenty groups here. The
Liu projection test and BAGofT reject at $p<0.05$, the others at $p\le0.05$. BAGofT pools the residuals
within groups it learns from the data and le Cessie's test over neighbourhoods in covariate space, so
both are listed with the pooled tests; le Cessie's test was run on the same data sets.
 The Liu projection test took a median of $17$ seconds a data set and BAGofT $371$.}
\label{tab:rivals-contam}
\begin{tabular}{lrrr}\hline
Test & clean & $\times4$ & $\times8$ \\ \hline
\multicolumn{4}{l}{\emph{pooled}} \\
\quad EDGE (default) & 0.080 & 0.020 & 0.050 \\
\quad EDGE, symmetric basis & 0.050 & 0.060 & 0.200 \\
\quad Hosmer--Lemeshow, $G=10$ & 0.020 & 0.000 & 0.060 \\
\quad BAGofT & 0.060 & 0.010 & 0.050 \\
\quad le Cessie--van Houwelingen & 0.070 & 0.040 & 0.070 \\
\multicolumn{4}{l}{\emph{record-level}} \\
\quad Liu projection test & 0.080 & 0.060 & 0.220 \\
\quad Stukel joint score & 0.060 & 0.450 & 0.490 \\
\quad Stukel one-parameter & 0.050 & 0.430 & 0.470 \\
\quad Stukel LR refit & 0.070 & 0.330 & 0.410 \\
\quad GiViTI belt & 0.070 & 0.290 & 0.370 \\
\quad cubic calibration LR & 0.060 & 0.350 & 0.400 \\
\hline\end{tabular}\end{table}


==> tables/tab_robust.tex <==
\begin{table}[htbp]\centering\small
\caption{Rejection rate at the nominal $5\%$ level under a correct logistic model with $k$
corrupted covariates, $n=1000$, when the model is fitted by maximum likelihood (ML) and by the
Huber-type quasi-likelihood estimator of \citet{cantoni2001robust} --- \textsf{robustbase}'s
\texttt{Mqle} at tuning constant $c=1.345$, with no weight on the covariates --- on the same
data. This study was run separately from that of
the main contamination table and on its own data sets, so its maximum-likelihood columns differ
from the corresponding rows of that table by Monte Carlo error alone. The robust fit converged in
all $1000$ replicates of every configuration and no replicate was excluded. With $k=0$ the
rates are sizes. The robust fit leaves every test's false-alarm rate where it was or raises
it, and it breaks the level of five of the ten tests the gate covers, even without contamination
--- Stukel's two score tests and three of the four forms of EDGE --- because their
reference is built on the maximum-likelihood information matrix. Only the default unit form of
EDGE, the two Hosmer--Lemeshow statistics, the belt and the cubic test are read
against a reference that still holds. Eleven tests were run and ten are shown: Stukel's
likelihood-ratio refit is omitted because a robust fit has no deviance, so under the robust arm
that refit compares a maximum-likelihood augmented fit against a robust base and is not a
likelihood-ratio test. $1000$ replicates; the nominal standard error is $0.007$.}
\label{tab:robust}
\begin{tabular}{lrrrrrr}\hline
 & \multicolumn{2}{c}{$k=0$} & \multicolumn{2}{c}{$k=10$} & \multicolumn{2}{c}{$k=25$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Test & ML & robust & ML & robust & ML & robust \\ \hline
EDGE (default) & 0.059 & 0.059 & 0.089 & 0.087 & 0.345 & 0.339 \\
EDGE, symmetric basis & 0.044 & 0.164 & 0.055 & 0.218 & 0.105 & 0.520 \\
EDGE, score-weighted & 0.056 & 0.619 & 0.659 & 0.560 & 0.899 & 0.737 \\
EDGE, symmetric score-weighted & 0.050 & 0.225 & 0.077 & 0.272 & 0.077 & 0.543 \\
Hosmer--Lemeshow & 0.059 & 0.050 & 0.045 & 0.063 & 0.114 & 0.171 \\
HL, Farrington-corrected & 0.059 & 0.051 & 0.046 & 0.059 & 0.116 & 0.140 \\
GiViTI belt & 0.049 & 0.054 & 0.379 & 0.400 & 0.639 & 0.678 \\
cubic calibration LR & 0.051 & 0.053 & 0.465 & 0.466 & 0.773 & 0.774 \\
Stukel joint score & 0.064 & 0.199 & 0.609 & 0.701 & 0.892 & 0.937 \\
Stukel one-parameter & 0.045 & 0.223 & 0.588 & 0.686 & 0.882 & 0.925 \\
\hline\end{tabular}\end{table}


==> tables/tab_tw.tex <==
\begin{table}[htbp]\centering\small
\caption{What protects a test. Rejection rate at $5\%$ on the same data sets, $1000$ replicates a row:
false alarms under a correct model, with $k$ records carrying the covariate multiplied by $4$ or $-4$
(shaded above $0.10$), and size-adjusted power under misfit (last six rows). EDGE at the default
partition and at ten groups; HL, the Hosmer--Lemeshow statistic at ten groups; HH, the weighted grouped
tests of Hosmer and Hjort with their general-purpose weight; Twin, the ungrouped score test for the
cubic directions of EDGE in the predicted risk; EDGE$_n$, EDGE with one record a group ($n\le1000$);
Spz, Spiegelhalter's $z$, whose raw rate is $0$ throughout and which is shown at its own realised level.}
\label{tab:tw}
\resizebox{\textwidth}{!}{\begin{tabular}{llrrrrrrrrrrrrr}\hline
Design & $n$ & Setting & EDGE & EDGE$_{10}$ & HL & HH$_{\mathrm{HL}}$ & HH$_{X^2}$ & Twin & EDGE$_n$ & Spz & Stukel & cubic & GiViTI \\ \hline
two covariates & 1000 & correct model & 0.063 & 0.059 & 0.052 & 0.055 & 0.055 & 0.057 & 0.057 & 0.050 & 0.063 & 0.058 & 0.049 \\
two covariates & 1000 & $\times4$, $k=1$ & 0.047 & 0.051 & 0.042 & 0.052 & 0.059 & \cellcolor{black!12}0.166 & \cellcolor{black!12}0.148 & \cellcolor{black!12}0.118 & \cellcolor{black!12}0.147 & \cellcolor{black!12}0.149 & \cellcolor{black!12}0.111 \\
two covariates & 1000 & $\times4$, $k=10$ & \cellcolor{black!12}0.101 & 0.066 & 0.049 & \cellcolor{black!12}0.183 & \cellcolor{black!12}0.271 & \cellcolor{black!12}0.641 & \cellcolor{black!12}0.594 & \cellcolor{black!12}0.546 & \cellcolor{black!12}0.595 & \cellcolor{black!12}0.454 & \cellcolor{black!12}0.375 \\
two covariates & 1000 & $\times-4$, $k=1$ & 0.051 & 0.041 & 0.043 & 0.073 & \cellcolor{black!12}0.141 & \cellcolor{black!12}0.468 & \cellcolor{black!12}0.379 & \cellcolor{black!12}0.303 & \cellcolor{black!12}0.378 & \cellcolor{black!12}0.393 & \cellcolor{black!12}0.278 \\
two covariates & 1000 & $\times-4$, $k=10$ & \cellcolor{black!12}0.406 & \cellcolor{black!12}0.210 & 0.093 & \cellcolor{black!12}0.676 & \cellcolor{black!12}0.815 & \cellcolor{black!12}0.992 & \cellcolor{black!12}0.986 & \cellcolor{black!12}0.987 & \cellcolor{black!12}0.986 & \cellcolor{black!12}0.978 & \cellcolor{black!12}0.966 \\
two covariates & 5000 & correct model & 0.049 & 0.050 & 0.027 & 0.037 & 0.038 & 0.052 & -- & 0.050 & 0.053 & 0.048 & 0.051 \\
two covariates & 5000 & $\times4$, $k=50$ & \cellcolor{black!12}0.745 & 0.096 & 0.069 & \cellcolor{black!12}0.456 & \cellcolor{black!12}0.615 & \cellcolor{black!12}0.989 & -- & \cellcolor{black!12}0.966 & \cellcolor{black!12}0.973 & \cellcolor{black!12}0.953 & \cellcolor{black!12}0.879 \\
two covariates & 5000 & $\times-4$, $k=25$ & \cellcolor{black!12}0.777 & \cellcolor{black!12}0.236 & \cellcolor{black!12}0.120 & \cellcolor{black!12}0.819 & \cellcolor{black!12}0.946 & \cellcolor{black!12}1.000 & -- & \cellcolor{black!12}1.000 & \cellcolor{black!12}1.000 & \cellcolor{black!12}1.000 & \cellcolor{black!12}1.000 \\
twelve covariates & 2000 & correct model & 0.045 & 0.065 & 0.050 & 0.065 & 0.070 & 0.057 & -- & 0.050 & 0.043 & 0.046 & 0.042 \\
twelve covariates & 2000 & $\times4$, $k=25$ & \cellcolor{black!12}0.102 & 0.055 & 0.054 & 0.061 & 0.072 & \cellcolor{black!12}0.218 & -- & \cellcolor{black!12}0.108 & \cellcolor{black!12}0.275 & \cellcolor{black!12}0.217 & \cellcolor{black!12}0.134 \\
twelve covariates & 2000 & $\times-4$, $k=10$ & 0.091 & 0.048 & 0.058 & 0.075 & 0.081 & \cellcolor{black!12}0.292 & -- & \cellcolor{black!12}0.134 & \cellcolor{black!12}0.315 & \cellcolor{black!12}0.306 & \cellcolor{black!12}0.204 \\
two covariates & 1000 & cloglog truth & 0.738 & 0.708 & 0.382 & 0.286 & 0.233 & 0.684 & 0.756 & 0.987 & 0.765 & 0.837 & 0.874 \\
two covariates & 1000 & top 2\%, risk 0.6 of prediction & 0.416 & 0.194 & 0.166 & 0.224 & 0.209 & 0.742 & 0.469 & 0.380 & 0.432 & 0.509 & 0.422 \\
two covariates & 1000 & C2, $k=10$ & 0.601 & 0.261 & 0.222 & 0.334 & 0.323 & 0.988 & 0.727 & 0.586 & 0.673 & 0.813 & 0.683 \\
two covariates & 5000 & top 2\%, risk 0.8 of prediction & 0.624 & 0.292 & 0.315 & 0.364 & 0.372 & 0.886 & -- & 0.661 & 0.578 & 0.718 & 0.526 \\
twelve covariates & 2000 & cloglog truth & 0.552 & 0.379 & 0.232 & 0.256 & 0.241 & 0.425 & -- & 0.225 & 0.545 & 0.622 & 0.614 \\
twelve covariates & 2000 & omitted interaction & 0.464 & 0.276 & 0.155 & 0.209 & 0.189 & 0.364 & -- & 0.260 & 0.490 & 0.483 & 0.587 \\
\hline\end{tabular}}\end{table}


==> tables/tab_twext.tex <==
\begin{table}[htbp]\centering\small
\caption{The same question on frozen predictions: rejection rate at $5\%$, $1000$ replicates a row,
on the corrupted data sets of the external-validation study ($n=1000$, five covariates), where nothing
is refitted. Twin, the score test for the cubic directions of EDGE in the frozen prediction, on three
degrees of freedom; Spz, Spiegelhalter's $z$; EDGE in external mode at ten groups and at the default
partition. Shaded above $0.10$.}
\label{tab:twext}
\begin{tabular}{lrrrrr}\hline
Setting & Twin & Spz & EDGE$_{10}$ & EDGE \\ \hline
correct model & 0.052 & 0.061 & 0.061 & 0.050 \\
$\times4$, $k=1$ & 0.061 & 0.048 & 0.044 & 0.055 \\
$\times4$, $k=2$ & 0.044 & 0.043 & 0.034 & 0.043 \\
$\times4$, $k=5$ & 0.067 & 0.054 & 0.059 & 0.072 \\
$\times4$, $k=10$ & 0.096 & 0.070 & 0.055 & 0.077 \\
$\times-4$, $k=1$ & 0.051 & 0.047 & 0.045 & 0.040 \\
$\times-4$, $k=2$ & 0.057 & 0.044 & 0.044 & 0.051 \\
$\times-4$, $k=5$ & \cellcolor{black!12}0.132 & 0.071 & 0.065 & \cellcolor{black!12}0.104 \\
$\times-4$, $k=10$ & \cellcolor{black!12}0.311 & 0.090 & 0.082 & \cellcolor{black!12}0.240 \\
\hline\end{tabular}\end{table}

